Multi-Sentence Grounding for Long-term Instructional Video

In this paper, we aim to establish an automatic, scalable pipeline for denoising the large-scale instructional dataset and construct a high-quality video-text dataset with multiple descriptive steps supervision, named HowToStep. We make the following contributions: (i) improving the quality of sentences in dataset by upgrading ASR systems to reduce errors from speech recognition and prompting a large language model to transform noisy ASR transcripts into descriptive steps; (ii) proposing a Transformer-based architecture with all texts as queries, iteratively attending to the visual features, to temporally align the generated steps to corresponding video segments. To measure the quality of our curated datasets, we train models for the task of multi-sentence grounding on it, i.e., given a long-form video, and associated multiple sentences, to determine their corresponding timestamps in the video simultaneously, as a result, the model shows superior performance on a series of multi-sentence grounding tasks, surpassing existing state-of-the-art methods by a significant margin on three public benchmarks, namely, 9.0% on HT-Step, 5.1% on HTM-Align and 1.9% on CrossTask. All codes, models, and the resulting dataset have been publicly released.

==> sec/3_method_backup.tex <==
\section{Method}
\label{sec:method}

In this section, our goal is to establish an automatic, scalable pipeline for ‘denoising’ the large-scale instructional dataset, and contribute a ‘cleaned’ video-text dataset, termed as \textbf{HowToStep}. 

\weidi{TO CONTINUE ...}

Specifically, we start by describing the problem scenario in \cref{subsec:problem}, including narration alignment and procedural step grounding. Then we present the proposed multi-sentence grounding network in \cref{subsec:network}. Lastly, we propose a novel pipeline to transform noisy and redundant ASR transcripts of instructional videos on the Internet into descriptive steps as an extra training source in \cref{subsec:pipeline}. 




%-------------------------------------------------------------------------
\subsection{Problem Scenario}
\label{subsec:problem}
 
Given an instructional video, $\mathcal{X}=\{\mathcal{V}, \mathcal{J}\}$, where $\mathcal{V} = \{V_1, V_2, \dots, V_T\}$ refers to the frames of the video, and $\mathcal{J} = \{J_1, J_2, \dots, J_K\}$ denotes the $K$ textual sentences (narrations or procedural steps) associated with the video. 
Our goal is to train a temporal multi-sentence grounding network that takes video and texts as inputs and outputs a textual-visual alignment score matrix ($\hat{\mathbb{A}}\in \mathbb{R}^{K \times T}$) with the binary visual alignability ($\hat{y}\in \mathbb{R}^{K\times 2}$) for each sentence. Formally, it can be denoted as:
\begin{align}
 \{\hat{y}, \hat{\mathbb{A}} \} = \Psi_{\text{align}}(\Phi_{\text{v-enc}}(\mathcal{V}), \Phi_{\text{t-enc}}(\mathcal{J}))
\end{align}
In training, the ground truth label $\mathbb{Y}_{\mathcal{J}\mathcal{V}} \in \{0, 1\}^{K \times T}$ takes value $\mathbb{Y}_{\mathcal{J}\mathcal{V}}^{[k,t]} = 1$ only if $k$-th text depicts what is happening in timestamp $t$ in the video, and zero otherwise. 

Depending on the type of given texts $\mathcal{J}\in\{\mathcal{N}, \mathcal{S}\}$, we differentiate the two targeted tasks as follows: 

\myparagraph{Narration alignment~\cite{han2022temporal}} 
\textbf{N}arrations $\mathcal{N}$ are textual sentences transcribed from the instructor's speech via the ASR system, which means these sentences have maintained a time order that can be utilized for visual grounding. Note that, some narrations are not visually alignable or not well-aligned with visual signals temporally as shown in \cref{fig:example}.


\myparagraph{Procedural step grounding~\cite{mavroudi2023learning}}
Procedural \textbf{S}teps $\mathcal{S}$ are collected from 
Wikihow~\cite{koupaee2018wikihow}, an external knowledge base with instructional articles explaining the procedures for completing certain tasks. Compared with narrations, the procedural steps do not necessarily have consistent temporal order as that happens in the video, or some steps may not even be present in the video at all. 
In addition, the training annotations $\mathbb{Y}_{\mathcal{S}\mathcal{V}}$ for this task are scarce.

% \weidi{we need to have a summary or discussion section, 
% to say, we can now train one model with ASR transcripts.
% however, they are sub-optimal, and what we do next to boost the current model, 
% with it as initial point.}
\myparagraph{Discussion} 
The ASR transcript with timestamps can be used as weakly-aligned labels $\mathbb{Y}_{\mathcal{N}\mathcal{V}}$ for training multi-sentence grounding network as previous work~\cite{han2022temporal}. However, 
as narrations essentially aim to assist people with hearing impairment, 
thus are not required to be descriptive of visual scenes,
and can be sometimes verbose with ambiguity. 
Training the grounding network to tackle both tasks only based on ASR transcripts is sub-optimal.
While on the other hand, procedural steps are concise and clear, that only contain the core actions to finish one specific task without redundancy. 
However, existing procedural steps, typically originating from the external knowledge base, are suitable for general scenarios but often differ from the specific steps depicted in the video.
Based on this observation, we first propose a pipeline to transform the noisy ASR transcripts into concise and descriptive steps for each instructional video, by exploiting the power of large language models~(LLMs), which effectively augment the dataset for training the grounding network, as detailed in the following subsection.

%---------------------------------------------------------------
\subsection{Architecture}
\label{subsec:network}

As shown in \cref{fig:arch}, 
we adopt a simple Transformer-based architecture, 
where visual features of each clip 
are individually encoded and treated as key-value pairs, 
the textual features of narrations or steps are treated as queries.
The queries iteratively attend visual features with cross-attention, 
and the alignment scores can be computed by textual-visual similarity, 
which emits high scores for any alignable sentences at their corresponding video timestamp. 
The following sections describe the full details.




\subsubsection{Visual-Textual Features} 
As defined in \cref{subsec:problem}, given an untrimmed long-form instructional video (6.7-mins long on average in our case) 
with $K$ associated texts (narrations or procedural steps), 
we compute the visual and textual features with pre-trained backbones, that can be denoted as: 
\begin{equation*}
    x_v = f(\mathcal{V}) \in \mathbb{R}^{T\times C}, \quad  x_j = g(\mathcal{J})\in \mathbb{R}^{K\times C}
    \label{eq:backbone}
\end{equation*}
where $x_v$ refers to features of a video sequence, and $x_j$ denotes the textual features for narrations or procedural steps associated with the video. $C$ is the dimension of the feature vector. Note that, the resulting feature dimensions depend on the pre-trained visual or textual backbone. 

We consider three popular pre-trained visual-language models, 
namely, the S3D-G backbone trained with MIL-NCE~\cite{xie2018rethinking, miech2020end}, CLIP-ViT/L-14 trained with InfoNCE~\cite{oord2018representation, radford2021learning, dosovitskiy2020image}, and InternVideo-MM-L14 trained with masked video
reconstruction and multi-modal contrastive loss~\cite{wang2022internvideo, wang2023videomae}. The ablation studies about these pre-trained backbones are presented in Sec. \ref{subsec:exp_ablation}.


\begin{figure}[!t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figs/network_12.pdf}
   \caption{Schematic visualization of the proposed Transformer-based multi-sentence grounding network termed \textbf{\modelname}.
   The visual features are treated as key-value pairs while textual features are treated as queries, to predict the alignment score matrix $\hat{\mathbb{A}}$ between video frames and texts.
   }
   \label{fig:arch}
\end{figure}


% \qirui{can we put the following 3 paragraphs about backbones into appendix?}

% \myparagraph{S3D-G}
% As for pre-processing, the video is decoded with 16 frames per second~(fps). Each 16-frame video clip cropped by a non-overlapping temporal window is fed into the S3D-G architecture, resulting in one feature~(512-d) per second. 
% For each sentence, it is encoded with the text encoder associated with the S3D-G video encoder~\cite{miech2020end}.
% Specifically, the sentence is first tokenized and converted into word vectors~(300-d) through an embedding layer trained on Google News. Then, word vectors from the same sentence will be projected into 512-d vectors, and turned into one sentence vector through maxpooling.


% \myparagraph{CLIP}~
% We decode the video into 1fps and extract one visual feature~(768-d) per second with OpenAI's ViT/L-14 model~\cite{dosovitskiy2020image}. The text feature~(768-d) is encoded with CLIP's text encoder. The embedding of the \texttt{<eot>} token is used as the feature for each sentence.


% \myparagraph{InternVideo}
% We decode the video into 8fps and feed it into the InternVideo-MM-L14 model with an 8-frame non-overlapping temporal window, obtaining one visual feature~(768-d) per second. The text encoder is the same as CLIP's but pre-trained on video-text datasets. Similarly, the embedding of the \texttt{<eot>} token is feature of each sentence.


\subsubsection{Multi-Sentence Grounding Module} 

As shown in \cref{fig:arch}, after extracting the visual and textual features independently, we project both features into the same dimension, fuse multimodal information with Transformer, and then predict the alignment score matrix between video and texts.

% \weidi{Give one short, simple sentence to lead this paragraph, for example, 
% As shown in Fig.~..... we do what ...}


\myparagraph{(1) Feature projection} 
After computing visual-textual features with pre-trained frozen models, we adopt one linear layer to project the features into the embedding with the same dimension $D$. In terms of positional encoding, we add sin/cos positional encoding to the visual features, while on the text side, we only add learnable positional embeddings to sentence features for the narration alignment task, but not in the step grounding task:
\begin{equation*}
    h_v = \phi_v(x_v)+p_v, \quad h_j = \phi_j(x_j)+\mathbb{I}_{\mathcal{J}=\mathcal{N}}\cdot p_j
    \label{eq:pe}
\end{equation*}
where $h_v \in \mathbb{R}^{T \times D}, h_j \in \mathbb{R}^{K \times D}$. $\phi_v, \phi_j$ refer to different projection heads for the features of video and sentences. $\mathbb{I}_{\mathcal{J}=\mathcal{N}}$ is the indicator function which takes value 1 only when input texts $\mathcal{J}$ are ordered narrations $\mathcal{N}$, otherwise zero. $p_v, p_j$ denote positional encoding for visual and textual features respectively. 


\myparagraph{(2) Visual-textual feature fusion} 
The visual features are processed with a temporal aggregator,
followed by a grounding module, expressed as:
\begin{equation*}
    o_v = \Phi_{\text{temp-agg}}(h_v), \quad o_j = \Psi_{\text{temp-ground}}(o_v, h_j)
    \label{eq:transformer}
\end{equation*}
where $o_v \in \mathbb{R}^{T \times D}, o_j \in \mathbb{R}^{K \times D}$, 
$\Phi_{\text{temp-agg}}(\cdot)$ refers to a temporal aggregator with three Transformer Encoder layers. $\Phi_{\text{temp-ground}}(\cdot)$ denotes a temporal grounding module, consisting of three Transformer Decoder layers, 
where visual features act as key-value pairs and textual features act as queries.

\myparagraph{(3) Alignment prediction}
In order to get the alignment score matrix between video and texts, 
we first project the output of the encoder and decoder into the same dimension,
\begin{equation*}
    z_v = \varphi_v(o_v) \in \mathbb{R}^{T \times d}, \quad z_j = \varphi_j(o_j) \in \mathbb{R}^{K \times d}
    \label{eq:proj}
\end{equation*}
% \weidi{insert the notation into the text description}
and then compute the alignment score matrix:
\begin{align*}
    \hat{\mathbb{A}}^{[k,t]} = \frac{{z_j^k} \cdot {z_v^t}^T}{\left\lVert z_j \right\rVert \cdot \left\lVert z_v \right\rVert} \in [0, 1]
    \label{eq:similarity}
\end{align*}
where $\hat{\mathbb{A}} \in \mathbb{R}^{K \times T}$ is the predicted alignment matrix. The higher value of $\hat{\mathbb{A}}^{[k,t]}$ means the $k$-th sentence is more likely to align with the visual content of timestamp $t$.






\subsubsection{Training Details} 
As introduced in \cref{subsec:problem}, 
given the ground truth labels $\mathbb{Y}_{\mathcal{J}\mathcal{V}}$, we train the multi-sentence grounding network with a variant of the InfoNCE loss, which has been adopted for such multi-sentence grounding problem~\cite{han2022temporal, mavroudi2023learning}:
\begin{equation*}
    \mathcal{L}= -\frac{1}{K}\sum^K_{k=1}\log \frac{\sum_t \mathbb{Y}_{\mathcal{J}\mathcal{V}}^{[k,t]}\exp(\hat{\mathbb{A}}^{[k,t]}/\tau)}{\sum_t\exp(\hat{\mathbb{A}}^{[k, t]}/\tau)}
    \label{eq:infonce}
\end{equation*}
where $\mathbb{Y}_{\mathcal{J}\mathcal{V}}\in \{0, 1\}^{K \times T}$ is the ground truth alignment matrix. 
$\tau$ is a temperature hyper-parameter, and $k, t$ refer to $k$-th sentence and $t$-th timestamp in the video respectively.


% \weidi{the clarification to be done in this whole Sec.~3.3:
% (i) again, terminology issue, description, narration, procedural steps, etc.
% (ii) the role of this section, and how the self-training initiates, for example, the reader is hard to get why we do this, may become clear after writing the dicussion in Sec.~3.2.}

%-------------------------------------------------------------------------

\begin{figure*}[!t]
  \centering
   \includegraphics[width=\linewidth]{figs/pipeline-resize_9.pdf}
   \vspace{-16pt}
   \caption{Schematic illustration of the proposed pipeline to summarizing redundant ASR transcripts into descriptive steps \textit{(left)}, while determining the start-end timestamp in the video \textit{(right)}. We utilize the large language model (LLM) to summarize the narrations from ASR transcripts into descriptive steps. Afterwards, we roughly get the pseudo-label by chaining the `steps$\rightarrow$transcript (ASR)' similarity and `transcript (ASR)$\rightarrow$video' timestamp to train our multi-sentence grounding network \textbf{\modelname} in \textbf{Stage 1}.
   Then we use the trained model to refine the timestamp of the generated steps in \textbf{Stage 2},
   resulting in an extra training source for multi-sentence grounding, named \textbf{HowToStep}.
   }
   \label{fig:pipeline}
   \vspace{-10pt}
\end{figure*}




\subsection{ASR Transcripts $\rightarrow$ Aligned \& Descriptive Procedural Steps}
\label{subsec:pipeline}

As presented in \cref{fig:pipeline}, 
the entire procedure can be divided into three parts: 
(i) we leverage LLM to summarize narrations from the ASR transcript into descriptive steps; (ii) we use the similarity between the original transcript and generated steps to roughly determine the start/end timestamp for each step as pseudo-label; 
(iii) we train the \textbf{\modelname} model on the generated steps with pseudo-label, and then use the trained model to refine the time range for each generated step (\ie, self-training). 
We name the final dataset as \textbf{HowToStep} and present the details in the following sections.

\subsubsection{Prompting LLM to Summarize Concise Steps}

To generate descriptive steps, 
we split the complete transcript for each video into $M$ segments, 
each segment $G_{i}$ consists of around 10 sentences.
Next, we prompt Llama2-7B~\cite{touvron2023llama} to summarize the transcripts into concise steps describing the main action presented in the video. Additionally, we prompt LLM to filter the colloquial sentences in the speech. We refer the readers to the complete prompt in \textbf{Appendix}. 

Formally, let $\Theta, \kappa$ refer to the large language model and the prompt texts, and the steps are generated separately:
\begin{equation*}
    \mathcal{S} = \{\hat{G}_1, \dots, \hat{G}_M\},  \text{\hspace{4pt}}  
    \hat{G}_i = \Theta  (G_i;\kappa),  \text{\hspace{3pt}} \forall i \in [1, M]
    \label{eq:prompt}
\end{equation*}
where $M$ is the number of separated ASR transcript segments. 
$\hat{G}_i$ refers to the summarized procedure steps for each segment $G_i$. 
$\mathcal{S}$ denotes the complete sequence of generated steps for one instructional video.
As a result, we have transformed the ASR transcripts of around 370k videos~(a subset of HowTo100M selected by~\cite{han2022temporal}) into approximately 7M descriptive procedural steps. 
For comparison, the Wikihow knowledge base only contains 100k procedural steps from 14k instructional articles, according to the statistics in~\cite{mavroudi2023learning}. 

\subsubsection{Temporal Grounding for LLM Generated Steps}
\label{subsubsec:2-stage}
We can simply get the desired steps grounding matrix between generated steps and video timestamps by directly computing $\mathbb{Y}_{\mathcal{S}\mathcal{V}}=g(\mathcal{S}) \cdot f(\mathcal{V})^T$, where $f(\cdot)$, $g(\cdot)$ is the corresponding visual-textual feature encoder. However, in practice, such an approach performs poorly, as shown in the ablation study at~\cref{tab:ablation_timestamp}.

Alternatively, after generating descriptive steps, 
we propose to acquire their corresponding temporal windows in the instructional videos, through a two-stage approach to determine the start/end timestamp.

\myparagraph{\indent Stage 1: Approximate estimation} 
As the procedural steps are summarized from transcripts (ASR), 
we first compute the similarity score between $S$ generated steps and $N$ narrations of the transcript from each video, 
getting `steps$\rightarrow$transcript' matrix:
\begin{equation*}
    \mathbb{T}_{\mathcal{S}\mathcal{N}} =  \text{softmax}(g(\mathcal{S}) \cdot g(\mathcal{N})^T/\nu, \text{dim}=1) 
\end{equation*}
where $\nu$ is temperature, $\mathbb{T}_{\mathcal{S}\mathcal{N}}\in \mathbb{R}^{S \times N}$ is the textual similarity matrix.
The generated steps grounding matrix can be computed by chaining the `steps$\rightarrow$transcript' 
and `transcript$\rightarrow$video' matrices, that has been defined in Sec.~\ref{subsec:problem}.
\begin{equation*}
    \mathbb{Y}_{\mathcal{S}\mathcal{V}} =  \mathbb{T}_{\mathcal{S}\mathcal{N}} \cdot \mathbb{Y}_{\mathcal{N}\mathcal{V}}, \quad \mathbb{Y}_{\mathcal{S}\mathcal{V}} \in \mathbb{R}^{S \times T}
\end{equation*}
We select the timestamp of the maximal alignment score as the centre time $c_k$ for each step $k$, 
\begin{equation*}
    c_k = \mathop{\text{argmax}}_t \mathbb{Y}_{\mathcal{S}\mathcal{V}}^{[k, t]}
\end{equation*}
and then find start-end timestamp ($s_k, e_k$) towards left and right side of $c_k$ until the alignment score ($\mathbb{Y}_{\mathcal{S}\mathcal{V}}^{[k, s_k]}, \mathbb{Y}_{\mathcal{S}\mathcal{V}}^{[k, e_k]}$) are lower than the percentage $\zeta$ of the score of the center time~(\ie, $\mathbb{Y}_{\mathcal{S}\mathcal{V}}^{[k, c_k]} \times \zeta$) following~\cite{mavroudi2023learning}. 
The step whose maximal alignment score $\mathbb{Y}_{\mathcal{S}\mathcal{V}}^{[k, c_k]}$ is lower than the threshold $\epsilon_1$ will be regarded as unalignable and discarded. 


% \weidi{say something like, Given neither `steps$\rightarrow$transcript' and `transcript$\rightarrow$video' matrix is perfect, 
% the alignment matrix between acquired procedure steps and video is naturally erroneous, we further propose to refine the temporal windows with self-training.}
% \weidi{I don't understand the last sentence, do you mean we train on the filtered ones, and inference on all, it would recycle some of the filtered ones back ?} \qirui{yes}
% \weidi{then say it.}

\myparagraph{\indent Stage 2: Temporal refinement} 
In the first stage, the start-end timestamp of the generated steps is completely obtained from weakly-aligned transcripts, 
which is naturally inaccurate, we further propose to refine the temporal windows by self-training.
As shown in \cref{fig:pipeline}, we train the proposed multi-sentence grounding network on the filtered steps with their temporal windows determined in the first stage as pseudo-labels. Then we use the trained model to do inference on the whole set of steps generated by LLM, to get new steps-to-video grounding matrix $\mathbb{Y}_{\mathcal{S}\mathcal{V}}$ for each video, which might recycle some of the filtered steps back.

As briefly described in \cref{subsec:problem}, 
when feeding video and a set of descriptive steps as input, 
the proposed \textbf{\modelname} model outputs the alignment matrix~($\hat{\mathbb{A}}$). We take the timestamp of the maximal alignment score as the start time for each step, and the duration is a constant $\vartriangle_{\text{sec}}$, following~\cite{chen2021multimodal, shvetsova2023howtocaption}. 
Similarly, the generated step with the maximal alignment score lower than the threshold $\epsilon_2$ will be discarded. Thus, we obtain a dataset consisting of aligned descriptive steps, named \textbf{HowToStep}. In practice, we observe that although our \textbf{\modelname} model is trained on noisy pseudo-labels~(\ie, relying on weakly-aligned transcripts, and getting steps-transcript similarity from imperfect language model), the model tends to learn the alignment patterns from procedural step to videos before overfitting to the noises, as also being observed in~\cite{zhang2021understanding}. 
More details for generating the dataset are presented in ablation studies in \cref{subsec:exp_ablation} and \textbf{Appendix}.

\myparagraph{Relation to existing work}
Generally speaking, the proposed idea here is similar to the recent work~\cite{mavroudi2023learning}, but with one crucial difference, that is, \cite{chen2022weakly, mavroudi2023learning, afouras2024ht} aims to ground steps collected from the only task-related articles in the external knowledge base~(\ie, Wikihow), 
while we try to align the descriptive steps summarized from the ASR transcript of the \emph{same} video. This design brings two benefits for training the multi-sentence grounding network: (i) the procedural steps generated per task are more diverse than those from Wikihow (\eg, 74 different videos are showing how to Make Pumpkin Puree in HowTo100M, while only one article of the same task is collected in Wikihow); 
(ii) the generated steps within the video are more likely to be alignable to the video itself than those externally sourced Wikihow steps naturally.




